Runtime Task Scheduling using Imitation Learning for Heterogeneous Many-Core Systems

Domain-specific systems-on-chip, a class of heterogeneous many-core systems, are recognized as a key approach to narrow down the performance and energy-efficiency gap between custom hardware accelerators and programmable processors. Reaching the full potential of these architectures depends critically on optimally scheduling the applications to available resources at runtime. Existing optimization-based techniques cannot achieve this objective at runtime due to the combinatorial nature of the task scheduling problem. As the main theoretical contribution, this paper poses scheduling as a classification problem and proposes a hierarchical imitation learning (IL)-based scheduler that learns from an Oracle to maximize the performance of multiple domain-specific applications. Extensive evaluations with six streaming applications from wireless communications and radar domains show that the proposed IL-based scheduler approximates an offline Oracle policy with more than 99% accuracy for performance- and energy-based optimization objectives. Furthermore, it achieves almost identical performance to the Oracle with a low runtime overhead and successfully adapts to new applications, many-core system configurations, and runtime variations in application characteristics.

==> acronyms.tex <==
\newacronym{TDP}{TDP}{thermal design power}
\newacronym[longplural={general-purpose processors}]{GPP}{GPP}{general-purpose processor}
\newacronym[longplural={no-operations}]{NOP}{NOP}{no-operation}
\newacronym{ILP}{ILP}{instruction-level parallelism}
\newacronym{VLIW}{VLIW}{very long instruction word}
\newacronym{DVFS}{DVFS}{dynamic voltage and frequency scaling}
\newacronym{DVS}{DVS}{dynamic voltage scaling}
\newacronym{DMR}{DMR}{dual modular redundancy}
\newacronym{HPC}{HPC}{high-performance computing}
\newacronym{DWC}{DWC}{duplication with comparison}
\newacronym{TMR}{TMR}{triple modular redundancy}
\newacronym{ROB}{ROB}{re-order buffer}
\newacronym{DSE}{DSE}{design space exploration}
\newacronym{TSH}{TSH}{tricriteria scheduling heuristics}
\newacronym{PG}{PG}{power gating}
\newacronym{CG}{CG}{clock gating}
\newacronym[longplural={functional units}]{FU}{FU}{functional unit}
\newacronym{PC}{PC}{program counter}
\newacronym{ECC}{ECC}{error correction code}
\newacronym[longplural={basic blocks}]{BB}{BB}{basic block}
\newacronym{BBHT}{BBHT}{basic block history table}
\newacronym{ASIC}{ASIC}{application-specific integrated circuit}
\newacronym{CMOS}{CMOS}{complementary metal-oxide-semiconductor}
\newacronym{ADPCM}{ADPCM}{adaptive differential pulse-code modulation}
\newacronym{DFT}{DFT}{discrete Fourier transform}
\newacronym{AVF}{AVF}{architectural vulnerability factor}
\newacronym{RTL}{RTL}{register-transfer level}
\newacronym{SET}{SET}{single-event transient}
\newacronym{SEU}{SEU}{single-event upset}
\newacronym{SBU}{SBU}{single bit upset}
\newacronym{MBU}{MBU}{multiple bit upset}
\newacronym[longplural={arithmetic logic units}]{ALU}{ALU}{arithmetic logic unit}
\newacronym{MMX}{MMX}{multimedia extension}
\newacronym{LUDCMP}{LUDCMP}{LU decomposition}
\newacronym{EDFP}{EDFP}{energy-delay-failure product}
\newacronym{EDP}{EDP}{energy-delay product}
\newacronym{ISA}{ISA}{instruction set architecture}
\newacronym{TCL}{TCL}{tool command language}
\newacronym{SEE}{SEE}{single-event effect}
\newacronym{DCT}{DCT}{discrete cosine transform} 
\newacronym{TLP}{TLP}{thread-level paralellism}
\newacronym{SRAM}{SRAM}{static random access memory}
\newacronym{FPGA}{FPGA}{field-programmable gate array}
\newacronym{ABFT}{ABFT}{algorithm-based fault tolerance}
\newacronym{TID}{TID}{total ionizing dose}
\newacronym{NMR}{NMR}{N-modular redundancy}
\newacronym{OoO}{OoO}{out-of-order}
\newacronym{VHDL}{VHDL}{VHSIC hardware description language}
\newacronym{DWP}{DWP}{duplicate when possible}
\newacronym{LANSCE}{LANSCE}{Los Alamos Neutron Science Center}
\newacronym{ACE}{ACE}{architecturally correct execution}
\newacronym{PPI}{PPI}{parallel programming interface}
\newacronym{OpenMP}{OpenMP}{open multi processing}
\newacronym{Pthreads}{Pthreads}{POSIX threads}
\newacronym{MPI}{MPI}{message passing interface}
\newacronym{FIFO}{FIFO}{first-in-first-out}
\newacronym{GCC}{GCC}{GNU compiler collection}
\newacronym{RAW}{RAW}{read after write}
\newacronym{MWPUETF}{MWPUETF}{mean work per unit of energy to failure}
\newacronym{MWTF}{MWTF}{mean work to failure}
\newacronym{LUT}{LUT}{look-Up table}
\newacronym{MITF}{MITF}{mean instructions to failure}
\newacronym{NASA}{NASA}{National Aeronautics and Space Administration}
\newacronym{CPU}{CPU}{central processing unit}
\newacronym{CFG}{CFG}{control flow graph}
\newacronym{MCCP}{MCCP}{multiple clustered core processor}
\newacronym{RMT}{RMT}{redundant multithreading}
\newacronym{IPC}{IPC}{instructions per cycle}
\newacronym{PID}{PID}{process ID}
\newacronym{DPM}{DPM}{dynamic power management}
\newacronym{MLP}{MLP}{multi-layer perceptron}
\newacronym{IPS}{IPS}{instructions per second}
\newacronym{NN}{NN}{neural network}
\newacronym{RC}{RC}{reconfiguration controller}
\newacronym{ML}{ML}{machine learning}
\newacronym{IL}{IL}{imitation learning}
\newacronym[longplural={systems-on-chip}]{SoC}{SoC}{system-on-chip}
\newacronym{WiFi-TX}{WiFi-TX}{WiFi transmitter}
\newacronym{WiFi-RX}{WiFi-RX}{WiFi receiver}
\newacronym{Range-Det}{Range-Det}{range detection}
\newacronym{SCT}{SCT}{single carrier transmitter}
\newacronym{SCR}{SCR}{single carrier receiver}
\newacronym{RT}{RT}{real-time}
\newacronym{RL}{RL}{reinforcement learning}
\newacronym{PMU}{PMU}{performance monitoring unit}
\newacronym{DAG}{DAG}{directed acyclic graph}
\newacronym{PAPI}{PAPI}{performance application programming interface}



==> algorithms/dagger_2.tex <==
\begin{algorithm}[tb]
\footnotesize
\SetNoFillComment
\caption{Hierarchical Imitation Learning Framework \todo{Option 2 - remove Algorithm 1 and Algorithm 2 and only keep this one (merged version)}} \label{algo:dagger}
\SetAlgoLined
\ForEach {task i in list\_of\_tasks $L$} {
$\mathcal{S}(i)$ = Get current state  \\
\tcc{\textbf{Level 1 - cluster selection}}
$C_i$ = $\bm{\pi_{C}}(\mathcal{S}(i))$ \\
\If {$C_i$ matches the Oracle decision $C_i^{*}$} {
    /* Proceed with execution */
}
\Else {
    Aggregate state $\mathcal{S}(i)$ and label $C_i^{*}$ to the dataset \\
}
\tcc{\textbf{Level 2 - PE selection}}
$\pi_{PE_{C}}$ $\leftarrow$  select the $\pi_{PE}$ of cluster $C_i$ \\
$PE_i$ = $\bm{\pi_{PE_{C}}}(\mathcal{S}(i))$ \\
\If {$PE_i$ matches the Oracle decision $PE_i^{*}$} {
    /* Proceed with execution */
}
\Else{
    Aggregate state $\mathcal{S}(i)$ and label $PE_i^{*}$ to the dataset \\
}
Assign task $i$ to $PE_i$
% t.PE $\leftarrow$ $PE_i$ 
}
\end{algorithm}

==> tables/feature_selection.tex <==
\begin{table}[tb]
\centering
\caption{Features employed for state representation}
\label{tab:feature_selection}
\begin{tabular}{@{}cclc@{}}
\toprule
\textbf{\begin{tabular}[c]{@{}c@{}}Feature\\ Type\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}Feature \\ Notation\end{tabular}} & \multicolumn{1}{c}{\textbf{\begin{tabular}[c]{@{}c@{}}Feature \\ Description\end{tabular}}} & \textbf{\begin{tabular}[c]{@{}c@{}}Feature\\ Categories\end{tabular}} \\ \midrule
\multirow{6}{*}{\textbf{Static}} & $t_{id}$ & ID of a task in the DAG & Task \\ \cmidrule(l){2-4} 
 & $T_{C_{i}}$ & \begin{tabular}[c]{@{}l@{}}Execution time of a task \\ in cluster $C_{i}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Task\\ PE\end{tabular} \\ \cmidrule(l){2-4} 
 & $D_{t_{i}}$ & Downward depth of task $t{i}$ & \begin{tabular}[c]{@{}c@{}}Task\\ Application\end{tabular} \\ \cmidrule(l){2-4} 
 & $t_{P_{i}}$ & Predecessor IDs of task $t{i}$ & \begin{tabular}[c]{@{}c@{}}Task\\ Application\end{tabular} \\ \cmidrule(l){2-4} 
 & A & Application Type & Application \\ \cmidrule(l){2-4} 
 & $P_{t_{i}}$ & \begin{tabular}[c]{@{}l@{}}Power consumption of a task\\ in cluster $C_{i}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Task\\ PE\end{tabular} \\ \midrule
\multirow{4}{*}{\textbf{Dynamic}} & $r_{job}$ & Relative job ID & Contention \\ \cmidrule(l){2-4} 
 & $C^{free}_{i}$ & \begin{tabular}[c]{@{}l@{}}Earliest time when PEs \\ in a cluster are ready \\ for task execution\end{tabular} & \begin{tabular}[c]{@{}c@{}}PE\\ Contention\end{tabular} \\ \cmidrule(l){2-4} 
 & $t_{P_{C_{i}}}$ & \begin{tabular}[c]{@{}l@{}}Clusters in which \\ predecessors executed\end{tabular} & \begin{tabular}[c]{@{}c@{}}Application\\ Contention\end{tabular} \\ \cmidrule(l){2-4} 
 & \multicolumn{1}{l}{$C_{t_{i}}^{t_{j}}$} & \begin{tabular}[c]{@{}l@{}}Communication time \\ from task $t_{i}$ to task $t_{j}$\end{tabular} & \begin{tabular}[c]{@{}c@{}}Task\\ Application\\ PE\\ Contention\end{tabular} \\ \bottomrule
\end{tabular}
\end{table}

==> tables/loo_dagger.tex <==
\begin{table}[tb]
\centering
\caption{Difference in average execution time with leave-one-out IL policies in comparison with Oracle}
\label{tab:loo_dagger}
\begin{tabular}{@{}rcc@{}}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{\begin{tabular}[c]{@{}c@{}}Applications excluded\\ from training\end{tabular}}}} & \multicolumn{2}{c}{\textbf{Policy}} \\ \cmidrule(l){2-3} 
\multicolumn{1}{c}{} & \multicolumn{1}{l}{\textbf{IL-LOO}} & \multicolumn{1}{l}{\textbf{IL-LOO-DAgger}} \\ \midrule
WiFi-TX & 123\% & 1.1\% \\ \midrule
WiFi-RX & 1467\% & 1.1\% \\ \midrule
Range Detection & 256\% & 1.4\% \\ \midrule
Single-Carrier TX & 127\% & 0.7\% \\ \midrule
Single-Carrier RX & 1165\% & 0.8\% \\ \midrule
Temporal Mitigation & 542\% & 1.3\% \\ \bottomrule
\end{tabular}
\end{table}

==> tables/soc.tex <==
\begin{table}[tb]
\centering
\caption{List of Processing Elements in the Many-Core Platform}
\label{tab:soc}
\begin{tabular}{@{}ccc@{}}
\toprule
\textbf{Cluster Name} & \textbf{Type} & \textbf{Number of Cores} \\ \midrule
\textbf{LITTLE} & General-Purpose & 4 \\
\textbf{big} & General-Purpose & 4 \\
\textbf{Matrix Multiplication} & Hardware Accelerator & 2 \\
\textbf{FFT} & Hardware Accelerator & 4 \\
\textbf{Viterbi} & Hardware Accelerator & 2 \\ \bottomrule
\end{tabular}
\end{table}

==> tables/workload.tex <==
\begin{table}[tb]
\centering
\caption{Number of jobs of each application in the workload used for experimental evaluation of the IL scheduler}
\label{tab:workload}
\begin{tabular}{@{}rc@{}}
\toprule
\multicolumn{1}{c}{\textbf{Applications}} & \textbf{Number of jobs in workload} \\ \midrule
WiFi-TX & 69 \\ \midrule
WiFi-RX & 111 \\ \midrule
Range Detection & 64 \\ \midrule
Single-Carrier TX & 64 \\ \midrule
Single-Carrier RX & 91 \\ \midrule
Temporal Mitigation & 101 \\ \bottomrule
\end{tabular}
\end{table}
